Towards Neural Synthesis for SMT-Assisted Proof-Oriented Programming

Proof-oriented programs mix computational content with proofs of program correctness. However, the human effort involved in programming and proving is still substantial, despite the use of Satisfiability Modulo Theories (SMT) solvers to automate proofs in languages such as F*. Seeking to spur research on using AI to automate the construction of proof-oriented programs, we curate a dataset of 600K lines of open-source F* programs and proofs, including software used in production systems ranging from Windows and Linux to Python and Firefox. Our dataset includes around 32K top-level F* definitions, each representing a type-directed program and proof synthesis problem producing a definition given a formal specification expressed as an F* type. We provide a program fragment checker that queries F* to check the correctness of candidate solutions. We also report on an extended version of our dataset containing a total of 940K lines of programs and proofs, with a total of 54k top-level F* definitions. We believe this is the largest corpus of SMT-assisted program proofs coupled with a reproducible program-fragment checker. Grounded in this dataset, we investigate the use of AI to synthesize programs and their proofs in F*, with promising results. Our main finding in that the performance of fine-tuned smaller language models (such as Phi-2 or StarCoder) compare favorably with large language models (such as GPT-4), at a much lower computational cost. We also identify various type-based retrieval augmentation techniques and find that they boost performance significantly. With detailed error analysis and case studies, we identify potential strengths and weaknesses of models and techniques and suggest directions for future improvements.

==> body/99.examples.tex <==
\section*{Interesting DT successes}

\begin{lstlisting}
let rec where #a #f (s:ordset a f) (c:condition a)
  : Pure (ordset a f)
       (requires True)
       (ensures fun (z:ordset a f) ->
           (as_list #a  z == FStar.List.Tot.Base.filter c 
            (as_list s)) /\
           (forall x. mem x z = (mem x s && c x)) /\
           (if size z > 0 && size s > 0 then 
            f (head s) (head z) else true))
  = match s with
    | [] -> empty
    | x::q -> 
      let z = where q c in
      if c x then insert' x z else z
\end{lstlisting}


\begin{lstlisting}[escapechar='']
FStar.Seq.Permutation.find

let rec find (#a:eqtype) (x:a) (s:seq a{ count x s > 0 })
  : Tot (frags:(seq a & seq a) {
      let s' = Seq.append (fst frags) (snd frags) in
      let n = Seq.length (fst frags) in
      s `Seq.equal` Seq.append (fst frags) (Seq.cons x (snd frags))
    }) (decreases (Seq.length s))
  = reveal_opaque (`%count) (count #a);
    if Seq.head s = x
    then Seq.empty, Seq.tail s
    else (
      let pfx, sfx = find x (Seq.tail s) in
      assert (Seq.equal (Seq.tail s)
                         (Seq.append pfx (Seq.cons x sfx)));
      assert (Seq.equal s
                         (Seq.cons (Seq.head s) (Seq.tail s)));
      Seq.cons (Seq.head s) pfx, sfx
    )
\end{lstlisting}


\begin{lstlisting}[escapechar='']

FStar.OrdMap.remove
val remove  : #key:eqtype -> #value:Type -> #f:cmp key -> key
              -> ordmap key value f -> Tot (ordmap key value f)
let remove #key #value #f x m =
  let s' = remove x (Mk_map?.d m) in
  let g' = F.on_dom key (fun (x':key) -> 
  if x' = x then None else (Mk_map?.m m) x') in
  Mk_map s' g'

\end{lstlisting}


\begin{lstlisting}[escapechar='']
FStar.Matrix.transposed_matrix_gen

val transposed_matrix_gen (#c:_) (#m:pos) (#n:pos) 
    (generator: matrix_generator c m n) 
  : (f: matrix_generator c n m { forall i j. f j i == generator i j })
let transposed_matrix_gen #c #m #n generator
  : (f: matrix_generator c n m { forall i j. f j i == generator i j })
  = fun j i -> generator i j
\end{lstlisting}


\begin{lstlisting}[escapechar='']
FStar.Monotonic.DependentMap.sel
val sel (#a:_) (#b:_)
    (r:map a b)
    (x:a)
  : Pure (option (b x))
    (requires True)
    (ensures (fun o -> DM.sel (repr r) x == o))
let rec sel #a #b
  (r:map a b)
  (x:a)
: Pure (option (b x))
  (requires True)
  (ensures (fun o -> DM.sel (repr r) x == o))
= match r with
  | [] -> None
  | (|k, v|)::tl -> if x = k then Some v else sel tl x
\end{lstlisting}


\begin{lstlisting}[escapechar='']
FStar.OrdSet.remove'
val remove': #a:eqtype -> #f:cmp a -> x:a -> s:ordset a f
    -> Tot (l:(ordset a f){ ((Nil? s ==> Nil? l) /\
        (Cons? s ==> head s = x ==> l = tail s) /\
        (Cons? s ==> head s =!= x ==> 
        (Cons? l /\ head l = Cons?.hd s)))})
let rec remove' #a #f (x:a) (s:ordset a f)
  : Tot (l:(ordset a f){ ((Nil? s ==> Nil? l) /\
                           (Cons? s ==> head s = x ==> l = tail s) /\
                           (Cons? s ==> head s =!= x ==> 
                           (Cons? l /\ head l = Cons?.hd s)))})
  = match s with
    | [] -> []
    | y::tl -> if y = x then tl else
               Cons?.hd s `insert'` remove' #a #f x tl
\end{lstlisting}


\begin{lstlisting}[escapechar='']
Pulse.Syntax.Base.eq_list
val eq_list (f: (x: 'a ->
    y: 'a -> b: bool{b <==> (x == y)})) (l m: list 'a)
    : b: bool{b <==> (l == m)}
let rec eq_list (f: (x: 'a -> 
    y: 'a -> b: bool { b <==> (x == y) } )) (l m: list 'a)
  : b: bool { b <==> (l == m) }
  = match l, m with
    | [], [] -> true
    | x::xs, y::ys ->
      f x y && eq_list f xs ys
    | _ -> false
\end{lstlisting}


\begin{lstlisting}[escapechar='']
Pulse.Syntax.Base.eq_opt
val eq_opt (f: (x: 'a -> 
    y: 'a -> b: bool{b <==> (x == y)})) (l m: option 'a)
    : b: bool{b <==> (l == m)}
let eq_opt (f: (x: 'a -> 
y: 'a -> b: bool{ b <==> (x == y) })) (l m: option 'a)
  : b: bool { b <==> (l == m) }
  = match l, m with
    | None, None -> true
    | Some x, Some y -> f x y
    | _ -> false
\end{lstlisting}


\begin{lstlisting}[escapechar='']
Hacl.Impl.MultiExponentiation.lexp_double_fw_consttime
val lexp_double_fw_consttime:
    #a_t:inttype_a
  -> len:size_t{v len > 0}
  -> ctx_len:size_t
  -> k:concrete_ops a_t len ctx_len
  -> l:size_window_t a_t len ->
  lexp_double_fw_st a_t len ctx_len k l
let lexp_double_fw_consttime 
    #a_t 
    len 
    ctx_len 
    k 
    l 
    ctx 
    a1 
    bLen 
    bBits b1 a2 b2 acc =
  [@inline_let]
  let table_len = 1ul <<. l in
  assert (v table_len == pow2 (v l));
  Math.Lemmas.pow2_le_compat (v l) 1;
  assert (1 < v table_len /\ v table_len * v len <= max_size_t);

  lexp_double_fw_gen len ctx_len k l table_len
    (lprecomp_get_consttime len ctx_len k l table_len)
    ctx a1 bLen bBits b1 a2 b2 acc
\end{lstlisting}


==> body/999.test.tex <==
\begin{minipage}{\textwidth}
  \begin{minipage}[b]{0.72\textwidth}
  \captionsetup{type=figure}
    \centering    
        \subcaptionbox{\centering Intra Project evaluation\label{subfig:test1}}[0.50\linewidth]{\includegraphics[width=.95\linewidth]{images/figures_rq1/class_compare_test.pdf}}%
        \subcaptionbox{\centering Intra Project evaluation\label{subfig:test2}}[0.50\linewidth]{\includegraphics[width=.95\linewidth]{images/figures_rq1/class_compare_test.pdf}}
    \captionof{figure}{\bf Verify@10 across different types of examples for different models.}
    \label{fig:test1}
  \end{minipage} \hfill
  \begin{minipage}[b]{0.27\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/rq1_errors/rq1_errors_3_category.pdf}
    \captionof{figure}{\bf Different errors spawned from the generated definitons by different models, presented as percentage of all errors. }
    \label{fig:test2}
    \end{minipage}
  \end{minipage}




==> body/rqs/rq4.tex <==
\subsection{Impact of Input Preparation.}
\label{sec:input_prep}

\input{tables/prompting_ablation}
\motivation

\experiment

\resultsec

% \analysis

\RS{4}{}


==> figures/rq3_errors.tex <==
\begin{figure}[tbh]
    \centering
\includegraphics[width=.8\linewidth]{images/rq3/rq3_errors_across_all.pdf}
    \caption{Errors made by models across different experimental setup}
    \label{fig:rq3-errors}
\end{figure}

==> includes/lstfstar.tex <==
\renewcommand\function{\ttfamily\color{dkblue}function}

\makeatletter
\lstdefinelanguage{fstar}{%
  basicstyle={\small\lst@ifdisplaystyle\scriptsize\fi},
  morekeywords=[1]{type,and,val,fun,let,in,ref,uref,mref,try,if,then,else,as,rec,assume,private,when,forall,assert,by_tactic,logic,array,pattern,effect,requires,ensures,decreases,modifies, abstract,total, reifiable, reflectable, new_effect, effect_actions, noeq, sub_effect, by, synth,splice,Pure,PURE,DIV,STATE,EXN,ALL,GHOST,Ghost,GTot,Lemma,Tot,Div,DIV,ST,St},
  morekeywords=[2]{WP, Post, Pre, Dv, TotST, M, Memo, READER, STATE_m, Effect, STEXN, RANDOM, MST, S_MST, MSTExn, TAC, Tac, TacH, Type},
  morekeywords=[3]{match,with,open, module, begin, end},
  morekeywords=[4]{},
  morestring=[b]",
  sensitive=true,%
  numbersep=4pt,
  % frame=none,
  backgroundcolor=\color{white},
%  numbers=left,
  columns=[l]fullflexible,
  texcl=true,
  mathescape=true,
%  xleftmargin=10pt,
  identifierstyle={\ttfamily},
  keywordstyle=[1]{\bf\ttfamily\maybecolor{dkblue}},
  keywordstyle=[2]{\bf\ttfamily\maybecolor{dkblue}},
  keywordstyle=[3]{\bf\ttfamily\maybecolor{dkpurple}},
  keywordstyle=[4]{\rmfamily\itshape},
% Here is the range marker stuff
  rangeprefix=(*---\ ,
  includerangemarker=false,
  stringstyle=\ttfamily,
  %lineskip=-2pt,
  showspaces=false,
  morecomment=[n]{(*}{*)},
  commentstyle={\ttfamily\itshape\maybecolor{dkgreen}},
  literate={->}{$\rightarrow\,$}{1}
           {True}{$\top$}{1}
           {False}{$\bot$}{1}
           {exists}{$\exists$}{1}
           {forall}{$\forall$}{1}
           {fun\ }{$\lambda$\ }{1}
           {~}{$\neg$}{1}           
           {~>}{$\leadsto$}{1}
           {`}{\`{}}{1}
           {'a}{$\alpha$}{1}
           {'b}{$\beta$}{1}
           {'c}{$\gamma$}{1}
           {`star`}{$\ast\,$}{1}           
           {-*}{$\mbox{--}\ast\,$}{1}                      
           {Gamma}{$\Gamma\,$}{1}
           {theta}{$\theta\,$}{1}
           {_0}{$_0$}{1}
           {_1}{$_1$}{1}
           {_2}{$_2$}{1}
           {_3}{$_3$}{1}
           {_4}{$_4$}{1}
           {/\\}{$\wedge\;$}{1}
           {\\/}{$\vee\;$}{1}
           {>=}{$\geq\ $}{2}
           {<=}{$\leq\ $}{2}
           {<==>}{$\Longleftrightarrow \ $}{3}
           {==>}{$\Longrightarrow \ $}{3}
           {|->}{$\mapsto \ $}{3}
           {<>}{$\neq$}{1}
           {--}{- }{1}   % Added due to         - not displaying properly.  Weird. ... but may make arrows look bad  {...}{$\ldots$}{3}
           {<<}{$\prec\ $}{1}
           {full_perm}{1.0}{1}    
           {forall_intro}{\tt forall\_intro}{1}
           {.Tot}{\tt .Tot}{1}
           ,
  breaklines=false}
\makeatother

